Value-Consistent Representation Learning for Data-Efficient Reinforcement Learning

Deep reinforcement learning (RL) algorithms suffer severe performance degradation when the interaction data is scarce, which limits their real-world application. Recently, visual representation learning has been shown to be effective and promising for boosting sample efficiency in RL. These methods usually rely on contrastive learning and data augmentation to train a transition model for state prediction, which is different from how the model is used in RL--performing value-based planning. Accordingly, the learned representation by these visual methods may be good for recognition but not optimal for estimating state value and solving the decision problem. To address this issue, we propose a novel method, called value-consistent representation learning (VCR), to learn representations that are directly related to decision-making. More specifically, VCR trains a model to predict the future state (also referred to as the ''imagined state'') based on the current one and a sequence of actions. Instead of aligning this imagined state with a real state returned by the environment, VCR applies a $Q$-value head on both states and obtains two distributions of action values. Then a distance is computed and minimized to force the imagined state to produce a similar action value prediction as that by the real state. We develop two implementations of the above idea for the discrete and continuous action spaces respectively. We conduct experiments on Atari 100K and DeepMind Control Suite benchmarks to validate their effectiveness for improving sample efficiency. It has been demonstrated that our methods achieve new state-of-the-art performance for search-free RL algorithms.

==> tables/ablation_atari_variants.tex <==
\begin{table*}[h]
\footnotesize % control font size
% \vspace{-4mm}
% \begin{table*}[h]
    % \footnotesize % control font size
    % \scriptsize
\centering
        \begin{adjustbox}{width=0.5\textwidth}
        \begin{tabular}{l c c c c}
            \toprule
            \textbf{Method} & \textbf{IQM}  & \textbf{optimality gap} \\
            \midrule
            Baseline                & 33.7 & 57.7            \\
            \shortname                & \textbf{39.7} & \textbf{54.4}             \\
            \midrule
            $d_\text{MSE}$                   &   30.9 & 60.0         \\
            $d_\text{MSE-A}$            &   34.0  & 57.9       \\
            % $d_\text{TD}$            & \textbf{39.7} & \textbf{54.3}    \\
            % \midrule
            % \shortnameno-NP             & \\
            \midrule
            SPR with reward loss    & 35.4  & 56.8\\
            SPR-L                   &  27.2  &  61.5 \\
            SPR-XL                  &  17.6  &  70.1 \\
            \midrule
            \shortname, $K=9$        & \textbf{39.7} & \textbf{54.3}     \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}

    % }
    % \vspace{-3.0pt}   % control the gap between the table bottom and next paragraph
    
\caption{A full list of all \ourname variants for ablation study.
% Here the table reports their aggregate results on Atari 100K. Baseline refers to SPR. $d_\text{MSE}$ and $d_\text{MSE-A}$ denotes another two value-consistent distance metrics.
% \emph{\shortnameno-NP } denotes that we don't use value consistency loss to update the policy learning network.
\emph{SPR with reward loss} denotes introducing an extra reward prediction part to SPR. \emph{SPR-L} and \emph{SPR-XL} denotes a modified SPR with 2x and 4x batch size for policy learning loss, keeping the batch size for RL loss unchanged. K represents prediction step. We increase K from 5 to 9, to see the influence on the performance.}
%\caption{Exploring the effect of the proposed cycle scheme on DM. \ourname-NG is the \ourname~ without the cycle loss updating on DM.}
\label{table:ablation_atari_variants}
    
\end{table*}
% \end{table*}
